Memory-efficient Continual Learning with Neural Collapse Contrastive

Contrastive learning has significantly improved representation quality, enhancing knowledge transfer across tasks in continual learning (CL). However, catastrophic forgetting remains a key challenge, as contrastive based methods primarily focus on "soft relationships" or "softness" between samples, which shift with changing data distributions and lead to representation overlap across tasks. Recently, the newly identified Neural Collapse phenomenon has shown promise in CL by focusing on "hard relationships" or "hardness" between samples and fixed prototypes. However, this approach overlooks "softness", crucial for capturing intra-class variability, and this rigid focus can also pull old class representations toward current ones, increasing forgetting. Building on these insights, we propose Focal Neural Collapse Contrastive (FNC^2), a novel representation learning loss that effectively balances both soft and hard relationships. Additionally, we introduce the Hardness-Softness Distillation (HSD) loss to progressively preserve the knowledge gained from these relationships across tasks. Our method outperforms state-of-the-art approaches, particularly in minimizing memory reliance. Remarkably, even without the use of memory, our approach rivals rehearsal-based methods, offering a compelling solution for data privacy concerns.

==> sections/main_paper.tex <==
%%%%%%%%% TITLE - PLEASE UPDATE
\title{Memory-efficient Continual Learning with Neural Collapse Contrastive}
%\title{Discovering  Hardness and Softness in Continual Learning through Neural Collapse Contrastive}%Discovering Hardness and Softness in Neural Collapse Continual Learning}

% \author{
%Trung-Anh Dang\textsuperscript{1},
%Vincent Nguyen\textsuperscript{1},
%Ngoc-Son Vu\textsuperscript{2},
%Christel Vrain\textsuperscript{1},\\
%\textsuperscript{1}LIFO - Université d'Orléans, France\\
%\textsuperscript{2}ETIS - CY Cergy Paris Université, ENSEA, CNRS, France\\
%{\tt\small trung-anh.dang@univ-orleans.fr, 
%{\tt\small vincent.nguyen@univ-orleans.fr, son.vu@ensea.fr, christel.vrain@univ-orleans.fr}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
%}
%}

\maketitle

%%%%%%%%% ABSTRACT
\begin{abstract}
    Contrastive learning has significantly improved representation quality, enhancing knowledge transfer across tasks in continual learning (CL). 
    % However, catastrophic forgetting remains a key challenge, as contrastive based methods primarily focus on ``soft relationships'' between samples that shift with data distribution changes, causing models to forget previously learned information. 
    However, catastrophic forgetting remains a key challenge, as contrastive based methods primarily focus on ``soft relationships'' or ``softness'' between samples, which shift with changing data distributions and lead to representation overlap across tasks. Recently, the newly identified Neural Collapse phenomenon has shown promise in CL by focusing on ``hard relationships'' or ``hardness'' between samples and fixed prototypes. However, this approach overlooks ``softness'', crucial for capturing intra-class variability, and this rigid focus can also pull old class representations toward current ones, increasing forgetting. Building on these insights, we propose Focal Neural Collapse Contrastive (FNC$^2$), a novel representation learning loss that effectively balances both soft and hard relationships. Additionally, we introduce the Hardness-Softness Distillation (HSD) loss to progressively preserve the knowledge gained from these relationships across tasks. Our method outperforms state-of-the-art approaches, particularly in minimizing memory reliance. Remarkably, even without the use of memory, our approach rivals rehearsal-based methods, offering a compelling solution for data privacy concerns.
    % However, catastrophic forgetting remains a key challenge, as contrastive based methods primarily focus on ``soft relationships'' between samples, which shift with changing data distributions and lead to overlap across tasks.
    
    %in memory-free scenarios, 
    % we do not compare with rehearsal-based methods in "memory-free setting"
    
    %Breakthrough advancements in contrastive learning have significantly improved representation quality, enabling better knowledge transfer across tasks in continual Learning. However, these methods still face catastrophic forgetting - the main challenge in continual learning when new information overlaps with previously learned knowledge. This problem occurs because these methods focus primarily on the relational information between samples (”Soft relationships” or “Softness”), which will always change when the data distribution shifts across tasks. Recently, a newly identified Neural Collapse phenomenon has been used and shown to perform well in continual Learning, by emphasizing learning “Hard relationships” or “Hardness” between samples and fixed class prototypes. However, this approach is not ideal for representation learning, since it overlooks “Softness”, which is crucial for capturing the distribution within each class, and an overly rigid approach may draw old class representations towards the present, potentially causing forgetting. Building on these observations, in this paper, we propose Focal neural collapse contrastive (FNC2), a novel representation learning loss that effectively integrates both soft and hard relationships. Additionally, we introduce the Hardness-Softness Distillation (HSD) loss to gradually preserve the knowledge gained from both types of relationships across previous tasks. With these proposed methods, the obtained performances are superior to state-of-the-art methods, especially in reducing memory dependence. Notably, in memory-free scenarios, our method performs comparably with rehearsal-based approaches, offering a solution to the problem of data privacy.%
\end{abstract}

%%%%%%%%% BODY TEXT
\section{Introduction}
\label{sec:intro}
Unlike human learning, which is adaptive and ongoing, current deep neural networks (DNNs) are typically trained in batches, using all available data at once. To emulate human learning, these models need to support continual learning (CL), which involves acquiring new knowledge while retaining previously learned information. However, this process is hindered by the phenomenon known as ``catastrophic forgetting'' (CF) \cite{mccloskey_1989, robins1995_catastrophic_fr}, where learning new tasks with fresh data causes the model to overwrite its prior knowledge, leading to a drastic decline in performance on older tasks. To tackle this challenge, CL has gained significant attention in recent years \cite{rusu_2016, co2l, dsdm_eccv_2022, wen2024provablecontrastivecontinuallearning, shiyaoli_tcp_wacv_2024, tang_kaizen_wacv_2024}. CL aims to develop methods that enable models to learn from a continuous stream of data by balancing the retention of prior knowledge with the ability to adapt to new information. Achieving this balance, known as the stability-plasticity trade-off, is crucial for preventing performance loss when integrating new tasks.

Current CL methods are predominantly based on supervised strategies, which have proven effective in preserving knowledge \cite{yoon_2018, buzzega2020darkexperiencegeneralcontinual, tiwari2022gcrgradientcoresetbased}. Notably, approaches that decouple representation learning from classifier training have shown greater resistance to forgetting compared to joint training methods \cite{co2l, fini2022cassle, madaan_2022_lump, wen2024provablecontrastivecontinuallearning}. Building on this decoupling, several supervised contrastive representation learning methods have delivered strong results \cite{co2l, wen2024provablecontrastivecontinuallearning}. However, \textcircled{1} most of these methods depend on replay buffers for storing past samples, limiting their use when data privacy is a concern. \textcircled{2} Another limitation is their reliance on inter-sample relationships, which can lead to \textit{\textbf{representation drift and overlap}} with new tasks—one of the main causes of forgetting in CL. Indeed, this issue has been highlighted in both DNNs \cite{yu_semantic_drift_2020, caccia2021_new_io_iclr} and neuroscience \cite{laura_drift_cl_neuroscience_2022}.

Neural collapse (NC), a recently discovered phenomenon characterized by highly structured and aligned neural network features, has attracted considerable attention in the deep learning community \cite{lu2021neuralcollapsecrossentropyloss, fang_pnas_2021, wenlong_ji_iclr_2022, han_nc_2021, tirer_extendeduf_2022, zhou_icml_2022}. It shows particular promise for CL by reducing representation overlap, enhancing class separation, and mitigating CF. NC achieves this by aligning feature representations with fixed prototypes, which act as optimal class-specific reference points and remain constant throughout training, significantly enhancing class separation. Additionally, prototypes can serve as class representatives, and their integration into contrastive learning reduces reliance on memory buffers. Leveraging these advantages, several CL methods \cite{yang2023neuralcollapse, yang2023neuralcollapseterminusunified, minhyuk_residual_2024} have incorporated NC. However, focusing only on sample-prototype relationships can reduce diversity, disrupt within-class data distribution, and lead to forgetting as older representations shift toward current task prototypes. To address this, we propose a supervised method using fixed, evenly spaced prototypes to enhance representation quality, minimize task overlap, and reduce memory dependence while preserving intra-class data distribution.

%Neural collapse (NC), a phenomenon characterized by structured and aligned neural network features, has recently attracted significant attention \cite{minhyuk_residual_2024, yang2023neuralcollapse, yang2023neuralcollapseterminusunified} for its potential to reduce representation overlap in CL. This is achieved by aligning feature representations with fixed prototypes that serve as optimal points for each class. As these prototypes remain unchanged throughout the learning process, class separation is significantly enhanced. Additionally, since prototypes can act as class representatives, incorporating them into contrastive learning can decrease the dependence on buffers. Leveraging these advantages, some CL methods \cite{yang2023neuralcollapse, yang2023neuralcollapseterminusunified} have employed this approach. However, since they focus only on sample-prototype relationships and ignore the relationships among samples, they encounter challenges of reduced diversity, disrupted within-class data distribution, and a tendency for old representations to shift toward current task prototypes, potentially leading to forgetting. Inspired by these works, we propose a supervised method that utilizes fixed, evenly spaced prototypes to enhance representation quality, minimize task overlap, and reduce memory dependence while preserving intra-class data distribution.

% Specifically, NC utilizes a fixed geometric structure where vertices represent prototypes mapped to specific classes.

To summarize, the main contributions of our work are:
% \begin{itemize}
%     \item We discover that the ``hardness'' (relationships between samples and fixed prototypes) and ``softness'' (relationships among samples) in NC-based methods play essential roles in both learning new tasks and preserving prior knowledge to obtain better invariant representations in continual learning.
%     \item We introduce a new plasticity loss, called Focal Neural Collapse Contrastive (FNC$^2$) loss, which effectively combines hardness and softness to enhance representation learning. This loss emphasizes hard samples while reducing the influence of easy samples during training.
%     \item To comprehensively preserve the knowledge from previous tasks, we propose a novel distillation loss called Hardness-Softness Distillation (HSD). HSD can consolidate both hard relations between samples and fixed equidistant prototypes and soft relationships (among samples), making the model significantly reduce forgetting when learning new tasks 
%     \item With the proposed methods, our models excel in both replay-based and memory-free scenarios. Specifically, in settings where no exemplars are stored, our model achieves state-of-the-art performance, enhancing its suitability for real-world applications that address data privacy concerns.
% \end{itemize}
\begin{itemize}
    \item We reveal that ``softness'' (inter-sample relationships) and ``hardness'' (relationships with fixed prototypes) \footnote{In unsupervised contrastive-based learning, \textit{alignment} ensures similar features are mapped to similar samples, while \textit{uniformity} ensures a feature distribution that maximizes information and ideally forms a uniform hypersphere. In a supervised setting, we use the term ``softness'' to represent alignment, and introduce ``hardness'' to describe the relationships between samples and NC-based prototypes.} are critical in NC-based contrastive CL for effectively acquiring new tasks while retaining prior knowledge.
    \item In both plasticity and stability phases of learning, we introduce new loss functions that address both hardness and softness. For plasticity, we propose Focal Neural Collapse Contrastive (FNC$^2$), a loss function that combines hard and soft semantics to enhance representation learning by focusing on challenging samples. For stability, we introduce the Hardness-Softness Distillation (HSD) loss function, which preserves knowledge from both hard and soft relationships, significantly reducing forgetting.
    %\item \textbf{Focal Neural Collapse Contrastive (FNC$^2$) loss:} We introduce FNC$^2$, a new plasticity loss that combines hardness and softness to improve representation learning. This loss emphasizes hard samples while reducing the influence of easy samples during training.
    %\item \textbf{Hardness-Softness Distillation (HSD):} To preserve knowledge from previous tasks, we propose a novel distillation loss called HSD. HSD can consolidates both hardness and softness, making the model significantly reduce forgetting when learning new tasks.
    \item Our model surpasses state-of-the-art (SoTA) results in both replay-based and memory-free scenarios, especially excelling in settings with no stored exemplars, making it ideal for applications with strict data privacy requirements.
\end{itemize}


%-------------------------------------------------------------------------
\section{Related Work}
\label{sec:related-work}
%-------------------------------------------------------------------------
\subsection{Continual Learning}
\label{sec:rw-continual-learning}
%\textbf{CL algorithms.} 

CL approaches can be broadly classified into three main categories. Rehearsal-based approaches \cite{madaan_2022_lump, buzzega2020darkexperiencegeneralcontinual,co2l, wen2024provablecontrastivecontinuallearning} store a small amount of data in a memory buffer and replay them to prevent forgetting. Regularization-based methods \cite{friedemann_si_2017, sangwon_neurips_2020, fini2022cassle, dongmin, tang_kaizen_wacv_2024} penalize changes in network parameters of the current task with respect to the previous task. Meanwhile, instead of using shared parameters, the architectural-based approaches \cite{rusu_2016, yoon_2018,li_learn_tg_2019} construct task-specific parameters and allow network expansion during CL. This work focuses on regularization-based methods by devising a specific regularization loss to align the current model with the previous one. Additionally, our approach is capable of performing well in both replay-based and memory-free scenarios.

%\textbf{Plasticity-stability trade-off vs. cross-task consilidation in CL.} 
Most of the current CL methods target primarily to achieve a balance between acquiring new tasks (\textbf{plasticity}) and retaining knowledge of previous tasks (\textbf{stability}) \cite{fini2022cassle, co2l, wen2024provablecontrastivecontinuallearning, szatkowski_wacv_2023}. To attain this balance, regularization-based approaches typically employ knowledge distillation (KD) \cite{hinton_kd_2015}, which aims to transfer knowledge from the previous trained model (teacher) to the current one (student). Recent works based on KD directly minimize the divergence between their intermediate representations \cite{hou_learning_2019} or final outputs \cite{fini2022cassle, pseudo_negative_icml_2024}. Additionally, several methods have explored relational KD, which enhances knowledge retention by leveraging the sample-to-sample relationships, such as Instance-wise Relation Distillation (IRD) \cite{co2l, wen2024provablecontrastivecontinuallearning}.
Other approaches, such as \cite{asadi_prd_cl_icml_2023, li_cl_important_sampling_2024}, focus on relationships between \textbf{\textit{learnable}} class prototypes and individual samples, rather than between samples themselves. 
In this work, we utilize KD through IRD, alongside a prototype-based distillation method. Our approach differs from \cite{asadi_prd_cl_icml_2023, li_cl_important_sampling_2024} in both the use of \textbf{\textit{fixed}} rather than learnable prototypes, and in how the sample-prototype relationships are applied.

% Additionally, several methods have explored relational KD, where knowledge retention is enhanced by leveraging the sample-to-sample relationships such as Instance-wise Relation Distillation (IRD) \cite{co2l, wen2024provablecontrastivecontinuallearning} or relationships between learnable class prototypes and samples as Prototype-Sample Relation Distillation (PRD)\cite{asadi_prd_cl_icml_2023}
% Early by minimizing the divergence between their intermediate representations \cite{hou_learning_2019} or final outputs \cite{fini2022cassle, co2l}. In this work, we utilize KD by focusing on distilling the final outputs through different relations related to current samples. 
Beyond balancing plasticity and stability, recent research emphasizes the importance of \textbf{cross-task} consolidation for improving representation and reducing forgetting \cite{lode_2023, osiris_zhang_2024}. In this work, we \textbf{\textit{implicitly}} address this by designing a plasticity loss function crafted to enhance the  cross-task separability.
% we are talking about cross-task consolidation 
%integration 





%-------------------------------------------------------------------------
\subsection{Contrastive Learning}
\label{sec:rw-contrastive-learning}
%Recently
Contrastive learning has emerged as a prominent representation learning approach, demonstrating its SoTA for different downstream tasks \cite{oord_representationlw_2018, simclr-chen20j, khosla2021supcon}. Numerous contrastive methods have been proposed and widely applied in both unsupervised \cite{oord_representationlw_2018, moco_v1_2020, chen2020_improved_bw, simclr-chen20j} and supervised settings \cite{khosla2021supcon}. 

In the context of CL, many studies \cite{fini2022cassle, scr_mai_2021, co2l, wen2024provablecontrastivecontinuallearning, li_cl_important_sampling_2024} have shown that contrastive learning is highly effective in acquiring task-invariant representations, which significantly mitigates the primary cause of forgetting — data imbalances between previous and current tasks. Among these, Co$^2$L \cite{co2l} is the first method to apply supervised contrastive learning in CL. Subsequently, CILA \cite{wen2024provablecontrastivecontinuallearning} improved Co$^2$L by analyzing the importance of coefficients for the distillation loss. Recently, CCLIS \cite{li_cl_important_sampling_2024} emerged as a SoTA method by preserving knowledge through importance sampling to recover previous data distributions. However, unlike Co$^2$L and CILA, CCLIS cannot operate without a memory buffer, which limits its efficiency in many real-world applications where data privacy is a concern.

Contrastive learning generates augmented views of each sample, bringing positive pairs closer and pushing negative pairs apart, promoting representation invariance to augmentations. Most contrastive methods focus on learning representations through relationships between samples, referred to as soft relationships or ``softness''. In CL, relying solely on softness preserves class diversity and data distribution but can cause task representation overlap, as shown in \cref{fig:comparasion-ours}a. In this paper, we propose a novel supervised contrastive loss for CL that reduces memory dependence and resolves this overlap while maintaining class distribution.

\begin{figure*}[t]
  \centering
   \includegraphics[width=0.8\linewidth]{images/compare_proto_diagram_14.pdf}

   \caption{Our method mitigates the drawbacks of both ``soft'' and ``hard'' learning by using fixed, equidistant prototypes to minimize cluster overlap. (a) Overlap between new and old classes happens due to non-fixed class clusters and representation drift. (b) Strong alignment with prototypes can overly cluster current task representations and pull older ones into new clusters, especially in CL with few old samples. Moreover, mixed-feature samples should be placed between classes, not tightly aligned with prototypes. (c) Our method considers both inter-sample and sample-prototype relationships, maintaining distinct cluster representations and preserving distribution within each cluster.}
   \label{fig:comparasion-ours}
\end{figure*}

%-------------------------------------------------------------------------
\subsection{Neural Collapse (NC)}
\label{sec:rw-neural-collapse}
A recent study \cite{papyan_2020} identified neural collapse (NC) phenomenon, where, at the end of training on a balanced dataset, class features collapse to their class means, aligned with a simplex equiangular tight frame (ETF). This finding has led to further research showing that NC represents global optimality in balanced training with cross-entropy \cite{lu2021neuralcollapsecrossentropyloss, florian_icml_2021, fang_pnas_2021, zhu_neurips_2021, wenlong_ji_iclr_2022} and mean squared error \cite{poggio_explicit_ra_2020, han_nc_2021, zhou_icml_2022, tirer_extendeduf_2022} loss functions. Inspired by NC, studies such as \cite{larue_nicolas_seeable_2022} have used fixed simplex ETF points with modified contrastive loss to achieve NC, while \cite{yang_induce_nc_2022} induced NC under imbalanced data conditions by fixing the classifier.

%A recent study \cite{papyan_2020} has identified a phenomenon called neural collapse (NC), in which, at the terminal phase of training on a balanced dataset, the features for each class collapse to their class mean, which are aligned with the vertices of a simplex equiangular tight frame (ETF). This discovery has motivated further research proving that NC is the global optimality of balanced training with cross-entropy \cite{lu2021neuralcollapsecrossentropyloss, florian_icml_2021, fang_pnas_2021, zhu_neurips_2021, wenlong_ji_iclr_2022} and mean squared error \cite{poggio_explicit_ra_2020, han_nc_2021, zhou_icml_2022, tirer_extendeduf_2022} loss functions. Inspired by NC, numerous studies have aimed to achieve this phenomenon by predefining the optimality and aligning the model accordingly. SeeABLE \cite{larue_nicolas_seeable_2022} demonstrated that utilizing a set of fixed points as a simplex ETF, with slight revisions to the contrastive loss function, can enable the model to reach NC, while \cite{yang_induce_nc_2022} induced NC under imbalanced data conditions by fixing the classifier. 

\textbf{Inducing NC for CL}. Building on \cite{galanti_ontr_2022}, which showed that NC persists when transferring models to new samples or classes, several CL studies have leveraged NC to mitigate forgetting \cite{yang2023neuralcollapse, yang2023neuralcollapseterminusunified}. These works pre-assign a group of classifier prototypes as a simplex ETF for all tasks and then align sample representations to their corresponding prototypes. The relationship between samples and prototypes, which this learning approach focuses on, is referred to as hard relationships, or ``hardness''. For instance, \cite{yang2023neuralcollapse, yang2023neuralcollapseterminusunified} employed the dot-regression (DR) loss proposed in \cite{yang_induce_nc_2022} for NC-based CL, which is considered a hard learning method. Since the prototype group remains consistent, these methods prevent task overlap but risk reducing diversity and disrupting within-class distribution, potentially leading to forgetting. Our method addresses this issue by integrating NC directly into the loss function, combining both softness and hardness to preserve data distribution and avoid task overlap in CL.

The concept of NC can be presented as follows.

\textbf{Definition 1.} A simplex Equiangular Tight Frame (ETF) is a collection of K vectors: $\mathbf{Q} = \{\mathbf{q}_k\}_{k=1}^{K}$, each vector $\mathbf{q}_k \in \mathbb{R}^{d}$, $K \le d+1$, which satisfies:

\begin{equation}
    \mathbf{Q} = \sqrt{\frac{K}{K-1}}\mathbf{U}\left(\mathbf{I}_K-\frac{1}{K}\mathbf{1}_K\mathbf{1}_K^T\right),
    \label{eq:etf}
\end{equation}
where $\mathbf{U} \in \mathbb{R}^{d \times K}$ is an orthogonal basis and $\mathbf{U}^{T}\mathbf{U}=\mathbf{I_K}$, $\mathbf{I}_K$ is an identity matrix and $\mathbf{1}_K$ is an all-ones vector.

Each vector $\mathbf{q}_k$ has the same $\ell_2$ norm, and any two distinct vectors consistently produce an inner product of $-\frac{1}{K-1}$, which is the lowest possible cosine similarity for K equiangular vectors in $\mathbb{R}^d$. This geometric relationship can be described as
\begin{equation}
    \mathbf{q}^T_{i}\mathbf{q}_{j}=\frac{K}{K-1}\delta_{i,j}-\frac{1}{K-1},\ \ \forall i, j\in[1,K],
    \label{eq:cosine-similarity-etf}
\end{equation}
where $\delta_{i, j}=1$ in case of $i=j$, and 0 otherwise.

After that, the NC phenomenon can be formally characterized by the following four attributes~\cite{papyan_2020}:

NC1: Features from the last layer within the same class converge to their intra-class mean, such that the covariance $\Sigma^{k}_V\rightarrow\mathbf{0}$. Here, $\Sigma^{k}_V=\mathrm{Avg}_{i}\{(\boldsymbol{\nu}_{k,i}-\boldsymbol{\mu}_{k})(\boldsymbol{\nu}_{k,i}-\boldsymbol{\mu}_{k})^T\}$, where $\boldsymbol{\nu}_{k,i}$ is the feature of sample $i$ in class $k$, and $\boldsymbol{\mu}_{k}$ is the intra-class feature mean.

NC2: After centering by the global mean, intra-class means align with simplex ETF vertices, i.e., $\{\tilde{\boldsymbol{\mu}}_k\}$, $1 \le k \le K$ satisfy \cref{eq:cosine-similarity-etf}, where $\tilde{\boldsymbol{\mu}}_k=(\boldsymbol{\mu}_k - \boldsymbol{\mu}_G) / \|  \boldsymbol{\mu}_k - \boldsymbol{\mu}_G \|$ and global mean $\boldsymbol{\mu}_G=\frac{1}{K}{\sum_{k=1}^{K}{\boldsymbol{\mu}_k}}$;

NC3:  Intra-class means centered by the global mean align with their classifier weights, leading to the same simplex ETF, i.e., $\tilde{\boldsymbol{\mu}}_k=\boldsymbol{w}_k/ \| \boldsymbol{w}_k \|$, where $1\le k \le K$ and $\boldsymbol{w}_k$ is the classifier weight of class $k$;

NC4: When NC1-NC3 hold, model predictions simplify to selecting the nearest class center, represented as $\text{argmax}_k\langle\mathbf{z}, \boldsymbol{w}_k\rangle=\text{argmin}_k||\mathbf{z}-\boldsymbol{\mu}_k||$, where $\langle \cdot , \cdot \rangle$ denotes the inner product operator, and $\mathbf{z}$ is the output of the model.

%Neural collapse reveals a specific geometric structure about the last layer feature and classifier 

%Neural collapse refers to a phenomenon at the terminal phase of training towards 0 train loss on balanced data \cite{papyan2020prevalence}. %A specific geometric structure emerges
%It reveals a geometric structure formed by the last-layer feature and classifier that can be defined as:


%Since this phenomenon enjoys  
% Due to the feature invariance within each class and the maximal equiangular separation among all class centers, neural collapse describes an optimal feature-classifier alignment status for classification. 


%Neural collapse corresponds to an optimal feature-classifier alignment for classification due to the maximized Fisher Discriminant Ratio (between-class variance to within-class variance). %From this perspective, we should keep this optimality for a model in problems that may break such alignment due to imperfect conditions such as imbalanced and incremental training. 

%can use it as an optimality to keep 

%-------------------------------------------------------------------------
\section{Preliminaries}
\label{sec:preliminaries}

%-------------------------------------------------------------------------
\subsection{Problem Setup}
\label{sec:problem-setup}

In the general supervised CL scenario, we have a sequence of training datasets, which is drawn from non-stationary data distributions for each task. Namely, let $t$ be the task index, where $t \in \{1,...,T\}$, and $T$ represents the maximum number of tasks. The dataset for the $t$-th task, denoted by $\mathcal{D}_t$, consists of $N_t$ supervised pairs: $\mathcal{D}_t=\{(\mathbf{x}_i,y_i)\}_{i=1}^{N_t}$, along with the set of classes $\mathcal{C}_t$. CL comprises a variety of scenarios; however, in this work, we focus specifically on two popular settings: class-incremental learning (Class-IL) and task-incremental learning (Task-IL). In both settings, there is no overlap in class labels across tasks, ensuring $\mathcal{C}_t \cap \mathcal{C}_{t'} = \emptyset$ for any two distinct tasks $t \neq t'$. For Task-IL, the learned model additionally has access to the task label during the testing phase.

%-------------------------------------------------------------------------
\subsection{Supervised Contrastive Learning}
This section details the SupCon algorithm \cite{khosla2021supcon}, which inspires the ``softness'' component of our approach. Suppose that in each batch $B$ of $N$ samples, SupCon firstly creates two randomly augmented versions of each sample in the batch, making each batch now contain $2N$ views: $\left|B\right|=2N$. After that, given the feature extractor $f$, each view $\mathbf{x}_i$ in the batch is mapped into a unit d-dimensional Euclidean sphere through a linear projector $g$ as $\mathbf{z}_i=h(\mathbf{x}_i)$, where $h = g \circ f$. Consequently, generic presentations are learned through the minimization of the following loss:
\begin{equation}
    \mathcal{L}_{SupCon}=\sum_{i=1}^{2N}\frac{-1}{\left|P(i)\right|}\sum_{j \in P(i)}\log(\frac{e^{\langle\mathbf{z}_i \cdot \mathbf{z}_j \rangle/\tau}}{\sum_{k \in A(i)}e^{\langle\mathbf{z}_i \cdot \mathbf{z}_k\rangle/\tau}})
    \label{eq:sup-con}
\end{equation}

% where $\langle\cdot,\cdot\rangle$ is the cosine similarity
where $\langle\cdot\rangle$ is the cosine similarity, $\tau > 0$ is the temperature factor, $A(i) = \{1..2N\} \setminus \{i\}$, and $P(i)$ is the index set of positive views with the anchor $\mathbf{x}_i$, denoted as:

\begin{equation}
    \label{eq:set-postive-index}
    P(i) = \{p \in \{1...2N\} | y_p=y_i, p \neq i\}    
\end{equation}

\noindent\textbf{Focal contrastive learning.} 
% Although contrastive learning methods have achieved outstanding performance in many applications for both supervised and unsupervised scenarios, their effectiveness in reducing intra-class feature dispersion remains limited. Indeed, contrastive learning highly relies on positive/negative pairs, but most of the samples are easy-to-contrast, leading to negligible contrastive loss gradients and causing intra-class samples to be scattered. To address this issue, drawing inspiration from focal loss~\cite{lin2018focallossdenseobject}, ~\cite{focalcontrastive} introduced the focal contrastive loss, described as
Despite their advantages, contrastive learning methods often struggle to reduce intra-class feature dispersion. They rely heavily on positive/negative pairs, but most samples are easy to contrast, resulting in minimal loss gradients and scattered intra-class samples. To address this issue, inspired by focal loss~\cite{lin2018focallossdenseobject}, ~\cite{focalcontrastive} introduced the focal contrastive loss. This approach emphasizes hard positive views—those with low cosine similarity to the anchor and thus lower prediction probability. Since hard positives are more influential in contrastive loss, they lead to clearer class clustering. Building on these insights, we propose focal contrastive loss in the context of NC for CL, as detailed in \cref{sec:fnc3}.

% described as
% \begin{equation}
%     \begin{split}
%         \mathcal{L}_{con}^{focal}=\sum_{i=1}^{2N}\frac{-1}{\left|P(i)\right|}\sum_{j \in P(i)}(1-u_{ij})\log(u_{ij}),
%     \end{split}
%     \label{eq:focal-con}
% \end{equation}
% where $u_{ij} = \frac{e^{\langle\mathbf{z}_i, \mathbf{z}_j\rangle/\tau}}{\sum_{k \in A(i)}e^{\langle\mathbf{z}_i, \mathbf{z}_k\rangle/\tau}}$. In \cref{eq:focal-con}, by adding the weight $(1-u_{ij})$, this loss 
% resulting in a low prediction probability $u_{ij}$.
%-------------------------------------------------------------------------
%\subsection{Neural Collapse Background}


%-------------------------------------------------------------------------
\section{Methodology}
\subsection{Motivation}
\label{sec:motivation}
Our method uses a two-stage learning process, as in ~\cite{co2l}. First, we learn a representation, which is then used to train the classifier. The main objective of CL is to balance two goals: learning new tasks (plasticity) and preserving the knowledge from previous tasks (stability). The overall loss can be described as:

\begin{equation}
    \label{eq:general-cl}
    \mathcal{L}_{overall}=\mathcal{L}_{plasticity} + \mathcal{L}_{stability}
\end{equation}

%where \(\mathcal{L}_{plasticity}\) is the plasticity loss of learning new knowledge, \(\mathcal{L}_{stability}\) is the stability loss of preserving previous knowledge.
\textbf{\textit{Remark.}} While plasticity and stability are central to most CL algorithms, some very recent works have highlighted the importance of cross-task consolidation \cite{lode_2023, osiris_zhang_2024}. Although our approach does not explicitly incorporate a cross-task consolidation term, we will show that it is implicitly accounted for in our $\mathcal{L}_{plasticity}$.

\noindent \textbf{a. Plasticity.} Previous contrastive learning approaches, like SupCon \cite{khosla2021supcon}, use sample relationships but allow class representations to shift, as shown in \cref{fig:comparasion-ours}a, causing overlap with current clusters and leading to forgetting. We term these methods ``soft plasticity''. To address this issue, inspired by Neural Collapse, recent works \cite{yang2023neuralcollapse, yang2023neuralcollapseterminusunified} propose using fixed, equidistant prototypes as the optimal class means at the end of training, as shown in \cref{fig:comparasion-ours}b. These methods, which we term ``hard plasticity'', focus on aligning sample representations with their assigned prototypes.

%In our work, we introduce novel methods of both plasticity learning and stability distillation. Firstly, we will illustrate the motivation for building our plasticity loss. In the supervised context, previous works in which their feature extractor are learning based on contrastive learning, only used the relation between samples by using some contrastive loss, such as SupCon \cite{khosla2021supcon} in supervised learning, which the representation of each class is not fixed, always change in each task as in \cref{fig:comparasion-ours}a. Consequently, these representations can overlap with current clusters in the current task, therefore leading to the forgetting, I denote these methods as soft learning. 
%To address this problem, inspired by Neural Collapse, some works \cite{yang2023neuralcollapse, yang2023neuralcollapseterminusunified} have proposed to pre-assigned the set of fixed equidistant prototypes in the feature space as the optimal class means at the end of the training, as visual in \cref{fig:comparasion-ours}b. After that, these works try to enforce the sample representation of each sample towards their corresponding prototypes, then I called this kind of method are hard learning. 

While these ``hard'' methods tightly align representations with prototypes, they have drawbacks. First, they neglect sample relationships, leading to representations clustered only around prototypes, which is not ideal since some samples share characteristics with multiple classes and should lie between them. Second, tightly aligning samples with current prototypes can pull old class representations towards the current task’s prototypes, causing forgetting, as shown in \cref{fig:comparasion-ours}b. To harness the benefits of NC while avoiding the pitfalls of hard learning, we propose to integrate both soft and hard learning. This approach maintains cluster distribution within each class and preserves separation from clusters of both current and past classes, as illustrated in \cref{fig:comparasion-ours}c.

%Although these methods make the representation of current tasks very tight with their prototype, they still have some drawbacks. Firstly, these methods pull too hard while ignoring the relation between samples, making the representation of the current sample only around their prototype, which is not for learning representation since some samples have characteristics of different classes, their representation should be in the space between all these classes, instead of only around very tight with their prototypes. Secondly, pulling too tight all samples to current prototypes also pulls the representation of old classes into the current task's prototype, causing the forgetting of old knowledge, as visualization in \cref{fig:comparasion-ours}c. To take advantage of the advantages of NC and overcome the disadvantages of hard learning, we propose a contrastive learning method that combines both soft learning and hard learning. With this new method for plasticity learning, the sample representations both maintain the distribution within each cluster and maintain the separation from the clusters of other classes in the current task as well as from the clusters of other classes in the past. 

\noindent  \textbf{b. Stability.} Co$^2$L, the pioneering work in continual contrastive learning, employs IRD as 
$\mathcal{L}_{stability}$.
The ``soft stability’’ IRD is designed to preserve the relationships between samples in the old and new feature spaces. However, as training progresses, its effectiveness diminishes, as demonstrated in \cref{fig:comare-ird-sprd}: 
\begin{enumerate}
    \item At the start of training task $t$, the representations of all current samples match those from task $t-1$ because no training has occurred yet. Initially, sample representations are consistent across tasks, but as training progresses, they gradually shift towards their respective class clusters.
    \item Over many epochs, the increasing discrepancy between the current and past feature spaces leads to a rise in IRD loss. This shift occurs because representations approach optimal positions, reducing the significance of 
$\mathcal{L}_{stability}$ based on IRD to the overall loss 
$\mathcal{L}_{overall}$ over time.
\end{enumerate} 
To address this limitation, we introduce a new distillation loss, termed ``hard stability’’, inspired by NC phenomenon, along with a novel strategy to enhance IRD's effectiveness throughout the training process. Both of these will be detailed in \cref{sec:hsd}.

As presented in \cref{fig:comparasion-ours}, both soft and hard learning methods suffer from representation drift, especially in settings with limited or no memory. Our approach effectively mitigates this issue. However, as the memory capacity increases, the impact of representation drift in soft and hard learning methods diminishes. Consequently, our method demonstrates a significant advantage in low-memory regimes, where the problem of representation drift is more pronounced.

\begin{comment}
 Besides, since the representation of the current task has separated from the previous task, we also introduce a novel distillation technique to preserve the past knowledge. In other previous work, there are many distillation techniques have been proposed, as in \cite{co2l} is the Instance-wise Relation Distillation (IRD), or through the output representation regularization as in \cite{fini2022cassle}. In both these distillation techniques, they all freeze the previous feature extractor for preserving past knowledge by using stop-gradient (denoted by $sg$). In this section, we will discuss why using IRD causes an increase in loss, and using only it is not an efficient way for distillation. The equation for IRD is described in \cite{co2l} as
\begin{equation}
    \label{eq:ird}
    \mathcal{L}_{IRD} = \sum_{i=1}^{2N}{-\mathbf{o}^{t-1}(\mathbf{x_i}) log(\mathbf{o}^{t}(\mathbf{x_i}))},
\end{equation}
where $\mathbf{o}^t(x_i)=[o^t_{i,1},...,o^t_{i,i-1},o^t_{i},o^t_{i,i+1},...,o^t_{i,K}]$, $|B|=2N$ is the number of samples each batch $B$, and each $o^t_{i,j}$ is described as
\begin{equation}
    \label{eq:ird-element}
    o_{i,j}^t=\frac{e^{<\mathbf{z_i}^t,\mathbf{z_j}^t>}}{\sum_{k\neq{i}}e^{<\mathbf{z_i}^t, \mathbf{z_k}^t>}},
\end{equation}
where $t$ is the task index, $t \ge 1$. Intuitively, IRD is used to distill the relation between samples in the batch in the old feature space and the new feature space. However, IRD reveals its limitations as the number of epochs increases during the training of new tasks, as shown in \cref{fig:comare-ird-sprd}. Specifically, at the beginning of training task t, representations of all samples in the current task are the same with their representations at task t-1, since there is no training at this time. When training starts, the representations of these samples move gradually into new positions, towards their corresponding class cluster. The relationship between the samples can be preserved in several epochs, but when the number of epochs is large, the difference in the current relation between sample representations in the current feature space increases compared to the past feature space, causing the value of IRD loss to increase. This increasing difference is because the learned representations are moving toward optimal positions near their prototypes. At this position, the relationship between the current samples is different from the relationship when they were at the beginning of training, causing the IRD distillation to be less meaningful than at the beginning. Based on the fact that the significance of IRD gradually decreases during training, we propose a new distillation loss function to maximize the effectiveness of IRD throughout the training process.   
\end{comment}




\begin{figure}[t]
  \centering
   \includegraphics[width=0.86\linewidth]{images/compare-ird-96.pdf}

   \caption{Shifts in representations of current samples at task $t$ between the beginning of training and after several epochs.}
   \label{fig:comare-ird-sprd}
\end{figure}


\subsection{Overview of the proposed method}
\begin{comment}
    

The overall of our methods can be described as in \cref{fig:overall-methods}. Our settings are described in \cref{sec:problem-setup} as in general continual learning setting. In our settings, the additional memory is optional because our methods have superior performance even in the memory-free case. In the case of storing old samples, we use the Reservoir sampling strategy \cite{reservoir_sampling_1985} to put samples into the fixed-size buffer, denoted as $\mathcal{M}$. After each task following the initial task, all current samples are combined with buffered samples, then each sample is independently drawn with equal probability in the mini-batch.

In our methods, we firstly predefined the set of fixed equidistant prototypes as the vertices of an Equiangular Tight Frame (ETF), which is created by using the algorithm as in \cref{eq:etf}. We denote this prototype set as $\mathbf{P} = \{\mathbf{p_i}\}_{i=1}^{K}$, $K$ is the number of prototypes, corresponding to the number of classes. These prototypes are then used as the equidistant optimal points in the feature space. We take full advantage of the value of these prototype points in both learning new tasks as well as distilling old tasks through direct use in the corresponding loss functions. In the following sections, I will present details about the plasticity loss functions in \cref{sec:fnc3} and stability loss in \cref{sec:hsd}.
\end{comment}
\cref{fig:overall-methods} provides an overview of our method (see \cref{sec:problem-setup} for setting details). 
% and even without it, our method outperforms other memory-based techniques. 
% and if old samples are stored, we use the Reservoir sampling strategy \cite{reservoir_sampling_1985} to fill a fixed-size buffer $\mathcal{M}$. 
In our approach, memory is optional, and when used, we employ the Reservoir sampling strategy \cite{reservoir_sampling_1985} to fill a fixed-size buffer $\mathcal{M}$. After each task beyond the first, current samples are combined with buffered samples, and each sample is drawn independently with equal probability for the mini-batch. We first predefine a set of fixed equidistant prototypes as the vertices of an ETF. %, which is created using the algorithm in \cref{eq:etf}.
We denote this prototype set as $\mathbf{P} = \{\mathbf{p_i}\}_{i=1}^{K}$, $K$ is the number of prototypes, corresponding to the number of classes. These prototypes are used as equidistant optimal points in the feature space. We utilize these prototype points in both learning new tasks and distilling old tasks through their direct use in the corresponding loss functions. 

The overall objective of our method is:
\begin{equation}
    \label{eq:final-objective}
    \mathcal{L} = \mathcal{L}_{FNC^2} + \mathcal{L}_{HSD}
\end{equation}
with details on each new loss function provided in the following sections.

% \textbf{Remark.} DISCUSS about the limitation of predefined number of class. Use the argument in FSCIL paper. Give some potential ideas to address this (mixture of prototypes...)
\begin{figure*}[t]
  \centering
   \includegraphics[width=0.9\linewidth]{images/overall_methods_5.pdf}

   \caption{\textbf{Overall architecture of our method.} Augmented samples from each batch are fed into the current model $f^t$ to learn new knowledge via $\mathcal{L}_{FNC^2}$ and the frozen previous model $f^{t-1}$ for distillation using $\mathcal{L}_{HSD}$. The buffer is optional, and NC-based prototypes are directly involved in both loss functions during training. }
   \label{fig:overall-methods}
\end{figure*}

% Augmented versions of all samples in each batch are fed into both the current model $f^t$ to learn new knowledge via $\mathcal{L}_{FNC^2}$ and the previous model $f^{t-1}$ for distillation using $\mathcal{L}_{HSD}$. 

% The weights of the previous model are not updated, as indicated by the use of stop-gradient (denoted as $sg$). Additionally, the buffer for storing old samples is optional, and our model performs well even without it.






%-------------------------------------------------------------------------
\subsection{Hardness-Softness Plasticity}
\label{sec:fnc3}
Inspired by NC phenomenon \cite{papyan_2020} and the concept of focal loss for addressing batch imbalance during training, we introduce a novel loss called Focal Neural Collapse Contrastive (FNC$^2$), defined as:
\begin{align}
    \mathcal{L}_{FNC^2} = -\sum_{i=1}^n \frac{1}{|P_i| + 1} \Bigg(& \sum_{\mathbf{z}_{j} \in P_i} (1-c_{ij})^{\gamma} \log(c_{ij}) \nonumber \\
    &+ (1-r_{ij})^{\gamma} \log(r_{ij}) \Bigg)
    \label{eq:fnc3-loss}
\end{align}

%In this paper, inspired by other works using neural collapse \cite{yang2023neuralcollapse, yang2023neuralcollapseterminusunified} and the idea of focal loss in handling the imbalance issue in each batch during training, we introduce the novel loss called Focal Neural Collapse Contrastive (FNC$^2$) loss as in \cref{eq:fnc3-loss}:
\begin{comment}
    
\begin{equation}
    \begin{split}
        \mathcal{L}_{FNC^3} = -\sum_{i=1}^n\left[\frac{1}{|P_i| + 1} ( &\sum_{z_{j} \in P_i} (1-c_{ij})^{\gamma}\log(c_{ij})\right.\\
        &+ (1-r_{ij})^{\gamma}\log(r_{ij}))]
    \end{split}
    \label{eq:fnc3-loss}
\end{equation}
\end{comment}
where
\begin{comment}
\begin{equation}
    c_{ij}=\frac{e^{\langle\mathbf{z}_i, \mathbf{z}_j\rangle/\tau}}{\sum_{k \neq i}{e^{\langle\mathbf{z}_i, \mathbf{z}_k\rangle/\tau}} + \sum_{\mathbf{p}_i \in \mathbf{P}_{1:t-1}}{e^{\mathbf{z}_i \cdot \mathbf{p}_i/\tau}}}
    \label{eq:c-ij}
\end{equation}
\end{comment} 
\begin{equation}
    c_{ij}=\frac{e^{\langle\mathbf{z}_i \cdot \mathbf{z}_j\rangle/\tau}}{\sum_{k \neq i}{e^{\langle\mathbf{z}_i \cdot \mathbf{z}_k\rangle/\tau}} + \underbrace{\sum_{\mathbf{p}_i \in \mathbf{P}_{1:t-1}}{e^{\langle{\mathbf{z}_i \cdot \mathbf{p}_i}\rangle/\tau}}}_{\text{cross-task}}}
    \label{eq:c-ij}
\end{equation}
\begin{equation}
    r_{ij}=\frac{e^{\langle\mathbf{z}_i \cdot \mathbf{p}_{\mathbf{z}_i}\rangle/\tau}}{\sum_{k \neq i}{e^{\langle\mathbf{z}_i \cdot \mathbf{z}_k\rangle/\tau}} + \sum_{\mathbf{p}_i \in \mathbf{P}_{1:t-1}}{e^{\langle\mathbf{z}_i \cdot \mathbf{p}_i\rangle/\tau}}}
    \label{eq:r-ij}
\end{equation}

Here, $P(i)$ is the set of positive indexes for each anchor, as defined in \cref{eq:set-postive-index}, $|P(i)|$ represents its cardinality, and $\gamma$ is the focusing hyperparameter. Additionally, $\mathbf{p}_{\mathbf{z}_i}$ is the prototype (specifically, the ETF vertex corresponding to label $y_i$), and $\mathbf{P}_{1:t-1}$ represents the set of prototypes used in all previous tasks.

Intuitively, for each sample in the current task, we pull positive samples closer to the anchor and push negative samples away, forming clusters that are then pulled towards their optimal prototypes, as shown in \cref{eq:c-ij} and \cref{eq:r-ij}. This approach helps the model learn both hardness and softness information. 

By incorporating $(1-c_{ij})^{\gamma}$ and $(1-r_{ij})^{\gamma}$, $\mathcal{L}_{FNC^2}$ emphasizes hard samples - those that are positive but far from the anchor or far from their prototype. These hard samples are crucial in contrastive learning, as they significantly affect intra-class sample distribution, unlike easy-to-contrast samples. A larger $\gamma$ further focuses the model on training from samples that are distant from their positive views and prototypes. To reduce reliance on memory, we use prototypes from previous tasks as representative points for past samples and include their cosine similarity with the anchor in $c_{ij}$ and $r_{ij}$. This allows our method to use old prototypes as negative points, similar to \textit{\textbf{cross-task consolidation}} as described in \cite{lode_2023, osiris_zhang_2024}, aiding in distinguishing between current and old classes. This approach effectively mimics stored samples and facilitates robust learning even without past task samples, serving as a form of \textbf{\textit{pseudo-replay}} where old prototypes are effectively reintroduced. We will present performance in both memory-based and memory-free settings in \cref{sec:results}.

When using memory, we employ an asymmetric version of this loss, where only current samples serve as anchors and buffer samples are used solely as negative points.

%Furthermore, in this loss, by adding $(1-c_{ij})^{\gamma}$ and $(1-r_{ij})^{\gamma}$, we can pay more attention into the hard samples - the samples are positive with the anchor but is far away and pay more attention into the anchor which is far away from its prototype. We focus more on these hard samples because they are crucial in contrastive learning. While most samples are easy-to-contrast, resulting in negligible contrastive loss gradients, hard samples significantly impact the scattering of intra-class samples. Besides, choosing a larger value of $\gamma$ would encourage the model to concentrate on training from the samples that are farther from their positive views via \cref{eq:c-ij} and farther from their corresponding prototypes through \cref{eq:r-ij}. Additionally, to minimize the dependence on memory, we consider the prototypes of previous tasks as the representative points for past samples and add the cosine similarity between them and the anchor to the $c_{ij}$ and $r_{ij}$ as in \cref{eq:c-ij} and \cref{eq:r-ij}. In this way, our method can leverage old prototypes as negative points, mimicking the role of samples in memory, and can learn well even without past task samples. We will report our performance in both using memory and memory-free settings in \cref{sec:results}. 

%In the case of using memory, we use the asymmetric version of this loss as in \cite{co2l}, since only the samples from the current are considered as the anchors, and the samples in the buffer are only used as the negative points.

%-------------------------------------------------------------------------
\subsection{Hardness-Softness Distillation}
\label{sec:hsd}
Our new distillation loss, which capitalizes on both hardness and softness plasticity during training, is described as:
\begin{align}
    \mathcal{L}_{HSD} &= (1 - \alpha) \underbrace{\sum_{i=1}^{2N}{-\mathbf{o}^{t-1}(\mathbf{x}_i) \log(\mathbf{o}^{t}(\mathbf{x}_i))}}_{\mathcal{L}_{IRD}}
    \nonumber \\
    &\quad + \alpha \underbrace{\sum_{i=1}^{2N} -\textbf{q}^{t-1}(\mathbf{x}_i;\mathbf{P}_{1:t}) 
\log(\textbf{q}^t(\mathbf{x}_i;\mathbf{P}_{1:t}))}_{\mathcal{L}_{S-PRD}}
    \label{eq:hsd}
\end{align}
\begin{comment}
\begin{align}
    \mathcal{L}_{HSD} &= (1 - \alpha) \mathcal{L}_{IRD} + \alpha \mathcal{L}_{S-PRD} \nonumber \\
    &= (1 - \alpha) \underbrace{\sum_{i=1}^{2N}{-\mathbf{o}^{t-1}(\mathbf{x_i}) \log(\mathbf{o}^{t}(\mathbf{x_i}))}}_{\mathcal{L}_{IRD}}
    \nonumber \\
    &\quad + \alpha \sum_{i=1}^{2N} -\textbf{q}^{t-1}(\mathbf{x_i};\mathbf{P}_{1:t}) 
    \log(\textbf{q}^t(\mathbf{x_i};\mathbf{P}_{1:t}))
    \label{eq:hsd}
\end{align}

\begin{equation}
    \mathcal{L}_{HSD} = (1 - \alpha) \mathcal{L}_{IRD} + \alpha \mathcal{L}_{S-PRD}\\
    \label{eq:hsd}
\end{equation}
\end{comment}
with $\alpha = max(0, \frac{e - e_0}{E})$, $e$ is the epoch index, $e_0$ is the number of epochs used for the warm-up period, and $E$ is the number of epochs (details are provided in the Appendix). 
%$we propose additionally the loss $\mathcal{L}_{S-PRD}$, which is as
\begin{comment}
\begin{equation}
    \label{eq:sprd}
    \mathcal{L}_{S-PRD}=\sum_{i=1}^{2N}{-\textbf{q}^{t-1}(\mathbf{x_i};\mathbf{P}_{1:t})log(\textbf{q}^t(\mathbf{x_i};\mathbf{P}_{1:t}))},
\end{equation}
\end{comment}
Here, $\mathcal{L}_{IRD}$ (used in \cite{co2l}) represents ``soft stability'' while the proposed Sample-Prototype Relation Distillation loss $\mathcal{L}_{{S-PRD}}$ embodies ``hard stability''.

In $\mathcal{L}_{IRD}$, $\mathbf{o}^t(\mathbf{x}_i)=[o^t_{i,1},...,o^t_{i,i-1},o^t_{i},o^t_{i,i+1},...,o^t_{i,K}]$, $|B|=2N$ is the number of samples each batch $B$, and each $o^t_{i,j}$ is: $o_{i,j}^t=\frac{e^{\langle\mathbf{z}_i^t \cdot \mathbf{z}_j^t\rangle/\kappa}}{\sum_{k\neq{i}}e^{\langle\mathbf{z}_i^t \cdot \mathbf{z}_k^t\rangle/\kappa}}$,
where $t \ge 1$ is the task index and $\kappa$ is the temperature hyperparameter.
In $\mathcal{L}_{{S-PRD}}$, $\mathbf{P}_{1:t} = \{\mathbf{p_i}\}_{i=1}^{K}$ represents the set of prototypes used from task $1$ to task $t$, $K$ is the number of used prototypes, $K = |\mathbf{P}_{1:t}|$. Besides, we have $\textbf{q}^t{(\mathbf{x}_i;\mathbf{P}_{1:t})}=[q^t_{i,1}, q^t_{i,2},...,q^t_{i,K}]$, and each ${q}_{i,j}^t$ is computed as: $q_{i,j}^t=\frac{e^{\langle\mathbf{z}_i^t \cdot \mathbf{p}_j\rangle/\zeta}}{\sum_{k=1}^{K}{e^{\langle\mathbf{z}_i^t \cdot \mathbf{p}_k\rangle/\zeta}}}$, given the temperature factor $\zeta$.

$\mathcal{L}_{S-PRD}$ preserves hardness by maintaining sample-prototype relationships, while $\mathcal{L}_{IRD}$ focuses on softness, capturing the evolving relationships between samples during learning. While $\mathcal{L}_{S-PRD}$ strongly preserves old knowledge by regularizing sample-prototype relationships, it may hinder learning if used exclusively, as it restricts the adaptation of representations. Early in training, $\mathcal{L}_{IRD}$ is crucial as it supports learning plasticity, while $\mathcal{L}_{S-PRD}$ is less effective. As training progresses and representations approach their prototypes, $\mathcal{L}_{S-PRD}$ becomes more beneficial, enhancing distillation.
That is the motivation behind the idea of combining $\mathcal{L}_{IRD}$ and $\mathcal{L}_{S-PRD}$ in $\mathcal{L}_{HSD}$ (Hardness-Softness Distillation) with weights that shift over time. After an initial warm-up period ($e_0$ epochs), we gradually decrease $\mathcal{L}_{IRD}$ and increase $\mathcal{L}_{S-PRD}$ to balance learning and information preservation effectively.

\begin{comment}  
With $\mathcal{L}_{{S-PRD}}$, we try to maintain the relationship between samples and all used prototypes. Since all prototypes are fixed, using this distillation can be considered an approach to preserve hardness information. In IRD, preservation can be understood as preserving softness - the soft relationship information between samples when the representation of the sample changes during the learning process. Meanwhile, using the S-PRD loss function will preserve the old knowledge more strongly than IRD, because it regularizes the relationships of each representation with fixed prototypes, instead of the relationships with other representations, which will change over time. However, because the distillation is so strong, using only S-PRD loss will hinder the learning of plasticity, causing the representations to be almost unlearned during the training process. On the other hand, as can be seen in \cref{fig:comare-ird-sprd}, at the beginning of the new task t, the representations of the current task will be close to the prototypes of the old task, if S-PRD is applied immediately from these epochs, the samples will be forced to these positions, unable to learn. From these observations, we see that IRD loss will play a more important role in the early epochs, then gradually decrease in effectiveness. Meanwhile, S-PRD does not play an important role in this early stage when it hinders the learning process, but after the learning process increases, when the representations are close to the prototypes - or their optimal average points, S-PRD plays an important role, which can replace IRD to make the distillation more effective. Therefore, we proposed the distillation loss function HSD, which is a combination of IRD and S-PRD with the weights of these two loss components gradually changing throughout the learning process as in \cref{eq:hsd}. Specifically, after $e_0$ epochs for the warm-up process, the backbone has gradually stabilized, and the representation of current task samples becomes closer to the corresponding prototypes. At that time, we will gradually reduce the weight of $\mathcal{L}_{IRD}$ and gradually increase the weight of $\mathcal{L}_{S-PRD}$, so that the distillation process becomes more efficient, preserving more information. 
\end{comment}

%-------------------------------------------------------------------------
\section{Experiments}
\label{sec:experiments}

%-------------------------------------------------------------------------
\subsection{Datasets and Implementation details}
\label{sec:datasets}
\noindent \textbf{Datasets.} As in other continual contrastive learning works, we use thee datasets: Seq-Cifar-10, Seq-Cifar-100, and Seq-Tiny-ImageNet for all experiments. We consider the class-IL and task-IL settings, described in \cref{sec:problem-setup}. Seq-Cifar-10 is created from Cifar-10 \cite{krizhevsky2009learning} and divided into five tasks with two classes for each task, Seq-Cifar-100 contains five tasks (20 classes/task) built from Cifar-100 \cite{krizhevsky2009learning}, and Seq-Tiny-ImageNet has 10 tasks (20 classes/task) built from Tiny-ImageNet \cite{le2015tinyiv}.

%-------------------------------------------------------------------------
%\subsection{Set-up}
\noindent \textbf{Implementation details.} We train our method using ResNet-18 \cite{resnet18} as the backbone, and we remove the last layer of the backbone as \cite{co2l, fini2022cassle}. Similar to previous works \cite{simclr-chen20j, zbontar2021barlowtwinsselfsupervisedlearning, co2l}, we add a two-layer projection MLP on top of the backbone, followed by ReLU activation functions to map the output of the backbone into $d$-dimension embedding space, where $d=128$ with Seq-Cifar-10 and Seq-Cifar-100, $d=256$ with Seq-Tiny-ImageNet. With a batch size of 512, we train the backbone with 500 epochs for the initial task and 100 epochs for other tasks as in \cite{co2l} for all datasets. Besides, we run with buffer sizes 0, 200 and 500 to evaluate the performance of the model with different memory settings. Regarding the value of $\gamma$ in $\mathcal{L}_{FNC^2}$, we choose $\gamma=1$ for Seq-Cifar-10, and $\gamma=4$ for all other datasets. Details about the selection of $\gamma$ and other hyperparameters are provided in the Appendix. Since Co$^2$L \cite{co2l} does not report results on Seq-Cifar-100 and results in the memory-free setting on Seq-Tiny-ImageNet, we run Co$^2$L on these cases for comparison. For evaluation, we train a classifier on top of the learned backbone using last-task samples and buffered samples with 100 epochs.

%-------------------------------------------------------------------------
\noindent \textbf{Evaluation metrics.} Similar to \cite{co2l, wen2024provablecontrastivecontinuallearning}, we evaluate the quality of the learned encoder $f^t$ by training a classifier $h^t$ on top of the frozen encoder $f^t$, using only the current training dataset $\mathcal{D}_t$ and the samples from the memory $\mathcal{M}$.
As defined in \cite{chaudhry_2018} as well as in other CL methods \cite{co2l, fini2022cassle, wen2024provablecontrastivecontinuallearning}, we compute the Average Accuracy (AA) on the test dataset and all accuracies $A_{T, k}$ of each task $k$ after learning the final task $T$. The equation for AA is defined as: 
\begin{equation}
    \label{eq:average-accuracy}
    AA = \frac{1}{T}\sum_{k=1}^{T}A_{T,k}
\end{equation}


\noindent\textbf{Considered methods.} To focus on learning ability with limited or no memory, we compare our method only with recent approaches that can operate in both settings. Since CCLIS \cite{li_cl_important_sampling_2024} and LODE \cite{lode_2023} cannot operate in memory-free scenarios, their results are excluded in \cref{tab:acc_result}. As shown in \cref{tab:memory-free-ability}, only Co$^2$L \cite{co2l}, the recent method CILA \cite{wen2024provablecontrastivecontinuallearning}, and ours can run without a memory buffer. Additionally, we compare our results with other well-known supervised methods, including ER \cite{riemer2019learninglearnforgettingmaximizing}, iCaRL \cite{rebuffi2017icarl}, GEM \cite{lopezpaz2017gem}, GSS \cite{aljundi2019gradientbasedsampleselection}, DER \cite{buzzega2020darkexperiencegeneralcontinual}, Co$^2$L \cite{co2l}, GCR \cite{tiwari2022gcrgradientcoresetbased}, and CILA \cite{wen2024provablecontrastivecontinuallearning}.





%-------------------------------------------------------------------------
\subsection{Main Results}
\label{sec:results}
\cref{tab:acc_result} reports results for buffer sizes 0 and 200 to highlight memory-free and limited memory scenarios. Results for a buffer size of 500 are provided in the Appendix. Although CILA \cite{wen2024provablecontrastivecontinuallearning} can operate without memory, results for this setting are not available due to the lack of publicly accessible code, so we cannot include them. 

As shown in \cref{tab:acc_result}, our model significantly outperforms recent replay-based methods across various CL settings, datasets, and buffer sizes. Notably, without using a buffer, our method outperforms Co$^2$L in all settings and datasets. For Seq-Cifar-10, our method exceeds Co$^2$L by approximately $10\%$ in Class-IL and $7.76\%$ in Task-IL. Similarly, for Seq-Cifar-100, our method outperforms Co$^2$L by $5.68\%$ for Class-IL and by $5.96\%$ for Task-IL. On Seq-Tiny-ImageNet, our method surpasses Co$^2$L in both Class-IL and Task-IL by $1.11\%$ and $3.6\%$, respectively. This improvement is less pronounced than on the CIFAR-10/100 datasets because the current evaluation protocol trains the classifier with samples from the current task and only a limited number from each old class. Consequently, the less significant improvements may stem from the classifier rather than the representation (we use a similar classifier training approach as others).

When compared to other methods with a memory buffer size of 200, our method outperforms all except for Seq-Cifar-100 in the Task-IL setting, where it lags behind GCR \cite{tiwari2022gcrgradientcoresetbased}. Notably, in the memory-free scenario, our method surpasses all replay methods with a buffer size of 200 on Seq-Cifar-10 and nearly matches the top result on Seq-Tiny-ImageNet, achieved by CILA. Although memory-free results for CILA are not available, our method outperforms their buffer size 200 results by 2.2\% on Seq-Cifar-10, highlighting its robustness in both limited memory and memory-free settings. With SoTA performance in memory-free scenarios, our model is well-suited for real-world applications where data storage is a concern.

Additionally, the Appendix includes average forgetting results to assess how well our method retains knowledge of previous tasks compared to other baselines.

\begin{table}
  \centering
  % {\small{

  % }}
    \resizebox*{!}{0.24\columnwidth}{
        \input{tables/table_memory_free_ability}
    }
  \caption{Among supervised CL, ours is one of the few that operates without memory.}
  \label{tab:memory-free-ability}
\end{table}

\begin{table*}[!t]
    \centering
    \resizebox*{!}{0.6\columnwidth}{
        \input{tables/table_acc_result}
    }
    \small
    \caption{Results for our method compared with other supervised baselines, with memory sizes 0 and 200, are averaged over five trials (best results in each column are highlighted in bold).}
    \label{tab:acc_result}
\end{table*}

\begin{comment}
\begin{table*}[!t]
    \centering
    \small
    \resizebox*{!}{1.1\columnwidth}{
        \input{table_forgetting}
    }
    \caption{Average Forgetting compared with all baselines in the supervised setting (lower is better). }
    \label{tab:add_forgetting_result}
\end{table*}
\end{comment}
%-------------------------------------------------------------------------
\subsection{Ablation Studies}
\label{sec:ablation-studies}
\noindent \textbf{Effectiveness of FNC$^2$.} To evaluate the efficiency of learning plasticity via $\mathcal{L}_{FNC^2}$, we compare it with the asymmetric version of SupCon loss ($\mathcal{L}_{SupCon}^{asym}$) \cite{co2l}, in combination with different using distillation methods scenario in the Class-IL setting. Note that with buffer size 0, the asymmetric loss $\mathcal{L}_{SupCon}^{asym}$ become the original SupCon loss ($\mathcal{L}_{SupCon}$). The results in \cref{tab:plasticity-verfication} show that when stability loss is absent, the performance with both $\mathcal{L}_{FNC^2}$ and $\mathcal{L}_{SupCon}^{asym}$ drops significantly, with both yielding approximately the same results. When using distillation methods, $\mathcal{L}_{FNC^2}$ outperforms $\mathcal{L}_{SupCon}^{asym}$ in all cases, especially in the case of no memory or small memory size (200).

\begin{table}
  \centering
  % {\small{

  % }}
    \resizebox*{!}{0.33\columnwidth}{
        \input{tables/table_ablation_plasticity}
    }
    \caption{Performance comparison of $\mathcal{L}_{FNC^2}$ with $\mathcal{L}_{SupCon}^{asym}$ in Class-IL setting on Seq-Cifar-10. The test $\mathcal{L}_{SupCon}^{asym}$ with $\mathcal{L}_{S-PRD}$ is omitted due to incompatibility, and in case of buffer size 0, $\mathcal{L}_{SupCon}^{asym}$ become $\mathcal{L}_{SupCon}$.}
    \label{tab:plasticity-verfication}
\end{table}

\noindent \textbf{Effectiveness of HSD.} In assessing the ability of $\mathcal{L}_{HSD}$ to preserve prior knowledge, we compare cases without and with different distillation methods, incorporating the plasticity loss $\mathcal{L}_{FNC^2}$. The results in \cref{tab:stability-verification} demonstrate that using either $\mathcal{L}_{IRD}$ \cite{co2l} or $\mathcal{L}_{S-PRD}$ individually yields minimal changes in performance. However, when both methods are combined in $\mathcal{L}_{HSD}$, performance consistently improves across all buffer sizes.


\begin{table}
  \centering
  % {\small{

  % }}
  \resizebox*{!}{0.47\columnwidth}{
    \input{tables/table_ablation_stability}
  }
  \caption{Ablation study on the effectiveness of $\mathcal{L}_{HSD}$ in class-IL. We run all tests on the Seq-Cifar-10 dataset with the plasticity loss $\mathcal{L}_{FNC^2}$ and different distillation methods.}
  \label{tab:stability-verification}
\end{table}

\noindent \textbf{Effectiveness of pseudo-replay prototypes.} We conduct ablation experiments using the class-IL setup on the Seq-Cifar-10 and Seq-Cifar-100 datasets with buffer size 0 and 200 to evaluate the role of pseudo-replay prototypes in our method. As shown in \cref{tab:pseudo-replay-verification}, this approach consistently improves performance across all datasets and buffer sizes. Notably, in the memory-free scenario, accuracy with pseudo-replay prototypes is close to that achieved with a buffer size of 200 without them. These outcomes validate our hypothesis that prior prototypes can act as effective representatives of past samples, enhancing cross-task consolidation when used as negative points in current tasks.   
\begin{table}
    \centering
    \resizebox*{!}{0.33\columnwidth}{
        \input{tables/table_ablation_pseudo_replay}
    }
    \caption{Influence of pseudo-replay prototypes.}
    \label{tab:pseudo-replay-verification}
\end{table}

\section{Conclusion}
\label{sec:conclusion}

We explore the roles of hard (``hardness'') and soft (``softness'') relationships in NC-based CL for both \textit{plasticity} and \textit{stability}. To address these, we propose two loss functions: $\mathcal{L}_{FNC^2}$ for plasticity, which uses fixed prototypes to guide representations towards optimal points while emphasizing hard samples and implicitly incorporating \textit{cross-task} consolidation through pseudo-replay of old prototypes, and $\mathcal{L}_{HSD}$ for distilling both hardness and softness over time. Our approach achieves SoTA in memory-free settings across various datasets and remains competitive with limited buffer sizes in memory-based scenarios.

\textbf{Limitations and future work.} Like other NC-inducing methods in CL, our approach is limited by the need to pre-define prototypes, which is impractical when the number of prototypes is unknown. In future work, inspired by recent advancements \cite{lu2024learningmixtureprototypesoutofdistribution}, we will tackle this issue by pre-defining a maximum number of prototypes and learning their distributions, allowing samples to be associated with multiple prototypes and different weights. Additionally, we plan to explore alternative memory-free evaluation methods, as current approaches including Co$^2$L \cite{co2l}, CILA \cite{wen2024provablecontrastivecontinuallearning} rely on buffers, which are less effective with limited samples for old classes. We also aim to identify easily forgotten samples and focus on distilling only the core knowledge.

% will also go deeper into finding out which samples have features that are easy to forget to focus on, instead of distilling the entire sample as currently. By distilling only the core knowledge that is often forgotten, we expect to improve the performance of the model in the continuous learning scenario.

% \textbf{Remark.} DISCUSS about the limitation of predefined number of class. Use the argument in FSCIL paper. Give some potential ideas to address this (mixture of prototypes...)

